Free Lunch in the Forest: Functionally-Identical Pruning of Boosted Tree Ensembles

Tree ensembles, including boosting methods, are highly effective and widely used for tabular data. However, large ensembles lack interpretability and require longer inference times. We introduce a method to prune a tree ensemble into a reduced version that is "functionally identical" to the original model. In other words, our method guarantees that the prediction function stays unchanged for any possible input. As a consequence, this pruning algorithm is lossless for any aggregated metric. We formalize the problem of functionally identical pruning on ensembles, introduce an exact optimization model, and provide a fast yet highly effective method to prune large ensembles. Our algorithm iteratively prunes considering a finite set of points, which is incrementally augmented using an adversarial model. In multiple computational experiments, we show that our approach is a "free lunch", significantly reducing the ensemble size without altering the model's behavior. Thus, we can preserve state-of-the-art performance at a fraction of the original model's size.

==> figures/ab-l1.tex <==
%\begin{adjustbox}{%
%    trim=15pt 0pt 0pt 15pt
%}
\begin{tikzpicture}
    \begin{axis}[
        width=0.95\linewidth,
        height=0.7\linewidth,
        enlargelimits=false,
        xmin=0,
        ymin=0,
        xmax=1005,
        ymax=200,
        grid=both,
        grid style={
            line width=.1pt,
            draw=gray!10
        },
        major grid style={
            line width=.2pt,
            draw=gray!50
        },
        minor tick num=4,
        xlabel={
            {Number of learners in the original ensemble \(M\)}
        },
        xlabel style={
            align=center,
            font={\scriptsize},
            %at={(axis description cs:0.5,-0.1)}
        },
        ylabel style={
            align=center,
            font={\scriptsize},
            %at={(axis description cs:-0.1,.5)}
        },
        ylabel={Number of learners in the\\pruned ensemble \(\left\| w \right\|_{0}\)},
        legend pos=outer north east,
        legend style={nodes={scale=0.6, transform shape}},
        legend cell align={left},
        legend image post style={scale=0.75},
        ticklabel style={
            font={\scriptsize}
        }
    ]
        \foreach\dataset in {%
            Breast-Cancer,%
            COMPAS,%
            ELEC2,%
            FICO,%
            HTRU2,%
            House-16H,%
            Ionosphere,%
            Pima-Diabetes,%
            PoL,%
            Seeds,%
            Spambase%
        } {%
            \addplot+[
                mark size=1.5pt,%
            ] table [
                discard if not={dataset}{\dataset},%
                x=n-fitted-estimators,%
                y=n-active-estimators,%
                col sep=comma%
            ] {csv/ab/l1/ab-l1.csv};
            \label{plot:\dataset}
        }
    \end{axis}
    \matrix[
        matrix of nodes,
        anchor=north,
        inner sep=0.1em,
        nodes={font=\scriptsize\sf},
        column 2/.style={anchor=base west},
        column 4/.style={anchor=base west},
        column 6/.style={anchor=base west},
        column 8/.style={anchor=base west},
    ] at([
        xshift=-1ex,
        yshift=-5.5ex
    ]current axis.south)
    {
        \ref{plot:Breast-Cancer} & Breast-Cancer &%
        \ref{plot:COMPAS} & COMPAS &%
        \ref{plot:ELEC2} & ELEC2 &%
        \ref{plot:FICO} & FICO &%
        \\
        \ref{plot:House-16H} & House-16H &%
        \ref{plot:HTRU2} & HTRU2 &%
        \ref{plot:Ionosphere} & Ionosphere &%
        \ref{plot:PoL} & PoL &%
        \\
        \ref{plot:Pima-Diabetes} & Pima-Diabates &%
        \ref{plot:Seeds} & Seeds &%
        \ref{plot:Spambase} & Spambase &%
        % & &%
        \\
    };
\end{tikzpicture}
%\end{adjustbox}

==> sections/0-links.tex <==
\begin{links}
    \link{Package}{www.github.com/eminyous/fipe}
    \link{Code}{www.github.com/eminyous/fipe-experiments}
    \link{Paper with appendices}{arxiv.org/abs/2408.16167}
\end{links}
